Sample Complexity of Robust Learning against Evasion Attacks

It is becoming increasingly important to understand the vulnerability of machine learning models to adversarial attacks. One of the fundamental problems in adversarial machine learning is to quantify how much training data is needed in the presence of evasion attacks, where data is corrupted at test time. In this thesis, we work with the exact-in-the-ball notion of robustness and study the feasibility of adversarially robust learning from the perspective of learning theory, considering sample complexity. We first explore the setting where the learner has access to random examples only, and show that distributional assumptions are essential. We then focus on learning problems with distributions on the input data that satisfy a Lipschitz condition and show that robustly learning monotone conjunctions has sample complexity at least exponential in the adversary's budget (the maximum number of bits it can perturb on each input). However, if the adversary is restricted to perturbing $O(\log n)$ bits, then one can robustly learn conjunctions and decision lists w.r.t. log-Lipschitz distributions. We then study learning models where the learner is given more power. We first consider local membership queries, where the learner can query the label of points near the training sample. We show that, under the uniform distribution, the exponential dependence on the adversary's budget to robustly learn conjunctions remains inevitable. We then introduce a local equivalence query oracle, which returns whether the hypothesis and target concept agree in a given region around a point in the training sample, and a counterexample if it exists. We show that if the query radius is equal to the adversary's budget, we can develop robust empirical risk minimization algorithms in the distribution-free setting. We give general query complexity upper and lower bounds, as well as for concrete concept classes.

==> sections/lb-local-queries.tex <==
\section{Local Membership Queries}


In this section, we show that the amount of data needed to $\rho$-robustly learn conjunctions under the uniform distribution has an exponential dependence on the adversary's budget $\rho$ when the learner only has access to the $\EX$ and $\LMQ$ oracles.
Here, the lower bound on the sample drawn from the example oracle is $2^\rho$, which is the same as the lower bound for \emph{monotone} conjunctions derived in \cite{gourdeau2022sample}, and the local membership query lower bound is $2^{\rho-1}$. 
%The constants before $\rho$ can be slightly altered with a trade-off between the two.
The result relies on showing there there exists a family of conjunctions that remain indistinguishable from each other on any sample of size $2^\rho$ and any sequence of $2^{\rho-1}$ LMQs with constant probability.


\begin{theorem}
\label{thm:conj-lmq-lb}
Fix a monotone increasing robustness function $\rho:\N\rightarrow \N$ satisfying $2 \leq \rho(n) \leq n/4$ for all $n$.
Then, for any query radius $\lambda$, any $\rho(n)$-robust learning algorithm for the class $\Conj$ with access to the $\EX$ and $\lambda$-$\LMQ$ oracles has  joint sample and query complexity lower bounds of $2^\rho$ and $2^{\rho-1}$ under the uniform distribution.
\end{theorem}

\begin{proof}
Let $D$ be the uniform distribution and WLOG let $\rho \geq 2$.
Fix two disjoint sets $I_1$ and $I_2$ of $2\rho$ indices in $[n]$, which will be the set of variables appearing in potential target conjunctions $c_1$ and $c_2$, respectively (i.e., their support).
We have $2^{4\rho}$ possible pairs of such conjunctions, as each variable can appear as a positive or negative literal.

Let us consider a randomly drawn sample $S$ of size $2^\rho$.
We will first consider what happens when all the examples in $S$ and the queried inputs $S'$ are negatively labelled.
Each negative example $x\in S$ allows us to remove at most $2^{2\rho+1}$ pairs from the possible set of pairs of conjunctions, as each component $x_{I_1}$ and $x_{I_2}$ removes at most one conjunction from the possible targets. 
By the same reasoning, each LMQ that returns a negative example can remove at most $2^{2\rho+1}$ pairs of conjunctions.
Note that the parameter $\lambda$ is irrelevant in this setting as each LMQ can only test one concept pair.
Thus, after seeing any random sample of size $2^\rho$ and querying any $2^{\rho -1}$ points, there remains 
\begin{equation}
\label{eqn:consistent-lmq}
\frac{2^{4\rho} - 2^{3\rho+1}-2^{3\rho}}{2^{4\rho}}\geq 1/4
\end{equation}
of the initial conjunction pairs that label all points in $S$ and $S'$ negatively. 
Then, choosing a pair $(c_1,c_2)$ of possible target conjunctions uniformly at random and then choosing $c$ uniformly at random gives at least a $1/4$ chance that $S$ and $S'$ only contain negative examples (both conjunctions are consistent with this).

Moreover, note that any  two conjunctions in a pair will have a robust risk lower bounded by $15/32$ against each other under the uniform distribution (see Lemma~\ref{lemma:rob-loss-mon-conj} in  Appendix~\ref{app:useful}).
Thus, any learning algorithm $\A$ with LMQ query budget $m'=2^{\rho-1}$ and strategy $\sigma:(\boolhc \times \set{0,1})^m\rightarrow(\boolhc \times \set{0,1})^{m'}$ (note that the queries can be adaptive) can do no better than to guess which of $c_1$ or $c_2$ is the target if they are both consistent on the augmented sample $S\cup\sigma(S)$, giving an expected robust risk lower bounded by a constant.
Letting $\E$ be the event that all points in both $S$ and $\sigma(S)$ are labelled zero, we get
\begin{align*}
\eval{c,S}{\risk_\rho^D(\A(S\cup\sigma(S)),c)}
&\geq \Prob{c,S}{\E}\eval{c,S}{\risk_\rho^D(\A(S\cup\sigma(S)),c)\given \E} \tag{Law of Total Expectation}
 \\
&\geq \frac{1}{4}\;\eval{c,S}{\risk_\rho^D(\A(S\cup\sigma(S)),c)\given \E}
\tag{Equation~\ref{eqn:consistent-lmq}} \\
&= \frac{1}{4}\cdot\frac{1}{2}\;\eval{S}{\risk_\rho^D(\A(S\cup\sigma(S)),c_1)+\risk_\rho^D(\A(S\cup\sigma(S)),c_2)\given \E} 
\tag{Random choice of $c$} \\
&\geq\frac{1}{8}\;\eval{S}{\risk_\rho^D(c_1,c_2)\given \E} \tag{Lemma~\ref{lemma:rob-triangle}}\\
&>\frac{1}{8}\cdot\frac{15}{32} \tag{Lemma~\ref{lemma:rob-loss-mon-conj}}\\
&=\frac{15}{256}
\enspace,
\end{align*}
which completes the proof.
\end{proof}


We use the term \emph{robustness threshold} from \cite{gourdeau2021hardness} to denote an adversarial budget function $\rho:\N\rightarrow\R$ of the input dimension $n$ such that if the adversary is allowed perturbations of magnitude $\rho(n)$, then there exists a sample-efficient $\rho(n)$-robust learning algorithm, and if the adversary's budget is $\omega(\rho(n))$, then there does not exist such an algorithm.
Robustness thresholds are distribution-dependent when the learner only has access to the example oracle $\EX$, as seen in \cite{gourdeau2021hardness,gourdeau2022sample}.
%Notably, in that setting, the robustness threshold of conjunctions under the uniform distribution is $\Theta(\log(n))$.
Now, since the local membership query lower bound  above has an exponential dependence on $\rho$, any perturbation budget $\omega(\log n)$ will require a sample and query complexity that is superpolynomial in $n$, giving the following corollary.

\begin{corollary}
The robustness threshold of the class $\Conj$ under the uniform distribution with access to $\EX$ and an $\LMQ$ oracle is $\Theta(\log(n))$.
\end{corollary}

The robustness threshold above is the same as when only using the $\EX$ oracle \cite{gourdeau2021hardness}.
Finally, since decision lists and halfspaces both subsume conjunctions, the lower bound of Theorem~\ref{thm:conj-lmq-lb} also holds for these classes.




\section{Local Equivalence Queries}

==> sections/monotone-conjunctions.tex <==
Monotone conjunctions are perhaps the simplest class of functions to study in learning theory.

+ Summary of results

+ PAC algorithm for monotone conjunctions 

+ Related work (mainly saeed's work with monotone conjunctions)

A conjunction $c$ over $\{0,1\}^n$ can be represented a set of literals $l_1,\dots,l_k$, where, for $x\in\X_n$, $c(x)=\bigwedge_{i=1}^k l_i$. 
For example, $c(x)=x_1\wedge\bar{x_2}\wedge{x_5}$ is a conjunction.
Monotone conjunctions are the subclass of conjunctions where negations are not allowed, i.e. all literals are of the form $l_i=x_j$ for some $j\in[n]$.

The standard PAC learning algorithm to learn monotone conjunctions is as follows.
We start with the hypothesis $h(x)=\bigwedge_{i\in I_h} x_i$, where $I_h=[n]$. 
For each example $x$ in $S$, we remove $i$ from $I_h$ if $c(x)=1$ and $x_i=0$. 

When one has access to membership queries, one can easily exactly learn monotone conjunctions over the whole input space: we start with the instance where all bits are 1 (which is always a positive example), and we can test whether each variable is in the target conjunction by setting the corresponding bit to 0 and requesting the label.

We refer the reader to \cite{mohri2012foundations} for an in-depth introduction to machine learning theory.


\section{An Adversarial Sample Complexity Lower Bound}


In this section, we will show that any robust learning algorithm for
monotone conjunctions under the uniform distribution must have an
exponential sample-complexity dependence on an adversary's budget
$\rho$.  This result extends to any superclass of monotone
conjunctions, such as CNF formulas, decision lists and halfspaces.  It
is a generalization of Theorem~13 in \cite{gourdeau2021hardness},
which shows that no sample-efficient robust learning algorithm exists
for monotone conjunctions against adversaries that can perturb
$\omega(\log(n))$ bits of the input under the uniform distribution.

The idea behind the proof is to show that, for a fixed constant $\kappa<2$, and sufficiently large input dimension, a sample of size $2^{\kappa\rho}$ from the uniform distribution won't be able to distinguish between two disjoint conjunctions of length $2\rho$. 
However, the robust risk between these two conjunctions can be lower bounded by a constant.
Hence, there does not exist a robust learning algorithm with sample complexity 
$2^{\kappa\rho}$ that works for the uniform distribution, and arbitrary input dimension and confidence and accuracy parameters.


Recall that the sample complexity of PAC learning conjunctions is
$\Theta(n)$ in the non-adversarial setting.  On the other hand, our
adversarial lower bound in terms of the robust parameter is super
linear in $n$ as soon as the adversary can perturb more than
$\log(\sqrt{n}))$ bits of the input.

\begin{theorem}
\label{thm:mon-conj}
Fix a positive increasing robustness function $\rho:\N\rightarrow\N$. 
For $\kappa<2$ and sufficiently large input dimensions $n$, any $\rho(n)$-robust learning algorithm for {\MonConj} has a sample complexity lower bound of $2^{\kappa\rho(n)}$ under the uniform distribution.
\end{theorem}

The proof of Theorem~\ref{thm:mon-conj} relies on the following lemmas:
\begin{lemma}[Lemma 6 in \cite{gourdeau2021hardness}]
\label{lemma:robloss-triangle}
Let $c_1,c_2\in\{0,1\}^\X$ and fix a distribution on $\X$. 
Then for all $h:\boolhc\rightarrow\set{0,1}$
\begin{equation*}
\robloss(c_1,c_2)
\leq \robloss(h,c_1)+\robloss(h,c_2)
\enspace.
\end{equation*}
\end{lemma}

We then recall the following lemma from \cite{gourdeau2021hardness}, whose proof here makes the dependence on the adversarial budget $\rho$ explicit.

\begin{lemma}
\label{lemma:bound-loss}
Under the uniform distribution, for any $n\in\N$, disjoint $c_1,c_2\in{\MonConj}$ of even length $3\leq l\leq n/2$  on $\boolhc$ and robustness parameter $\rho= l/2$, we have that $\robloss(c_1,c_2)$ is bounded below by a constant that can be made arbitrarily close to $\frac{1}{2}$ as $l$ (and thus $\rho$) increases. 
\end{lemma}
\begin{proof}
For a  hypothesis $c\in{\MonConj}$, let $I_c$ be the set of variables in $c$.
Let $c_1,c_2\in\C$ be as in the theorem statement.
Then the robust risk $\robloss(c_1,c_2)$ is bounded below by 
\begin{equation*}
\Prob{x\sim D}{c_1(x)=0\wedge x\text{ has at least $ \rho $ 1's in }I_{c_2}}\geq (1-2^{-2\rho})/2\enspace.
\end{equation*}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:mon-conj}]
Fix any algorithm $\A$ for learning {\MonConj}.
We will show that the expected robust risk between a randomly chosen target function and any hypothesis returned by $\A$ is bounded below by a constant.
%Fix a function $\poly(\cdot,\cdot,\cdot,\cdot,\cdot)$, and note that, since $\text{size}(c)$ and $\rho$ are both at most $n$, we can simply consider a function $\poly(\cdot,\cdot,\cdot)$ in the variables $1/\epsilon,$ and $1/\delta,n$ instead.
Let $\delta=1/2$, and fix a positive increasing adversarial-budget function $\rho(n)\leq n/4$ ($n$ is not yet fixed).
Let $m(n)=2^{\kappa\rho(n)}$ for an arbitrary $\kappa<0$.
Let $n_0$ be as in Lemma~\ref{lemma:concepts-agree}, where $m(n)$ is the fixed sample complexity function. 
Then Equation~(\ref{eqn:sample-size}) in the proof of Lemma~\ref{lemma:concepts-agree} holds for all $n\geq n_0$.
%Set such a $n$ that also satisfies $l\leq n/2$ and $l\geq 3$. 

Now, let $D$ be the uniform distribution on $\boolhc$ for $n\geq \max(n_0,3)$, and choose $c_1$, $c_2$ as in Lemma~\ref{lemma:bound-loss}.
Note that $\robloss(c_1,c_2)>\frac{5}{12}$ by the choice of $n$.
Pick the target function $c$ uniformly at random between $c_1$ and $c_2$, and label $S\sim D^{m(n)}$ with $c$.
By Lemma~\ref{lemma:concepts-agree}, $c_1$ and $c_2$ agree with the labeling of $S$ (which implies that all the points have label $0$) with probability at least~$\frac{1}{2}$ over the choice of $S$. 

Define the following three events for $S\sim D^m$: 
\begin{align*}
&\E:\;{c_1}_{|S}={c_2}_{|S}\;,\enspace
\E_{c_1}:\;c=c_1\;,\enspace
\E_{c_2}:\;c=c_2\enspace.
\end{align*}

Then, by Lemmas~\ref{lemma:concepts-agree} and~\ref{lemma:robloss-triangle}, 

\begin{align*}
\eval{c,S}{\robloss(\A(S),c)}
&\geq\Prob{c,S}{\E}\eval{c,S}{\robloss(\A(S),c)\;|\;\E}\\
&>\frac{1}{2}(
\Prob{c,S}{\E_{c_1}}\eval{S}{\robloss(\A(S),c)\;|\;\E\cap\E_{c_1}}\\
&\qquad+\Prob{c,S}{\E_{c_2}}\eval {S}{\robloss(\A(S),c)\;|\;\E\cap \E_{c_2}}
)\\
&=\frac{1}{4}\;\eval{S}{\robloss(\A(S),c_1)+\robloss(\A(S),c_2)\;|\;\E}\\
&\geq \frac{1}{4}\;\eval{S}{\robloss(c_2,c_1)}\\
&=\frac{5}{48}
\enspace.
\end{align*}

\end{proof}




The proof of the theorem follows similar reasoning as Theorem~13 in
\cite{gourdeau2021hardness}, and is included in
Appendix~C.  The main difference in the proof is its
reliance on the following lemma, which shows that, for sufficiently
large input dimensions, a sample of size $2^{\kappa\rho}$ from the
uniform distribution will look constant with probability $1/2$ if
labelled by two disjoint monotone conjunctions of length $2\rho$.  As
shown in Lemma~14, which can be found in
Appendix~C, these two conjunctions have a robust risk
bounded below by a constant against each other.

\begin{lemma}
\label{lemma:concepts-agree}
For any constant $\kappa<2$, for any robustness parameter $\rho\leq n/4$, for any disjoint monotone conjunctions $c_1,c_2$ of length $2\rho$, there exists $n_0$ such that for all $n\geq n_0$, a sample $S$ of size $2^{\kappa\rho}$ sampled i.i.d. from $D$ will have that $c_1(x)=c_2(x)=0$ for all $x\in S$ with probability at least $1/2$.
\end{lemma}


\begin{proof}
We begin by bounding the probability that $c_1$ and $c_2$ agree on an
i.i.d. sample of size $m$.  We have
\begin{equation}
\label{eqn:zero-label-sample}
\Prob{S\sim D^m}{\forall x\in S  \cdot c_1(x)=c_2(x)=0}
%&=\left(\Prob{x\sim D}{x\in X_{00}}\right)^m\\
=\left(1-\frac{1}{2^{2\rho}}\right)^{2m}
\enspace.
\end{equation}
In particular, if 
%Bounding the RHS below by $1/2$, we get that, as long as 
\begin{equation}
\label{eqn:sample-size}
m\leq \frac{\log(2)}{2\log(2^{2\rho}/(2^{2\rho}-1))}
\enspace,
\end{equation}
then the RHS of  Equation~\ref{eqn:zero-label-sample} is at least $1/2$.

Now, let us consider the following limit, where $\rho$ is a function of the input parameter $n$:
\begin{align*}
\underset{n\rightarrow\infty}{\lim}\;
2^{\kappa\rho}\log\left(\frac{2^{2\rho}}{2^{2\rho}-1}\right)
&=\frac{-\log(4)}{\kappa\log(2)}\;\underset{n\rightarrow\infty}{\lim}\;\frac{2^{\kappa\rho}}{1-2^{2\rho}}   \\
&=\frac{-\log(4)}{\kappa\log(2)}\;\frac{\kappa\log(2)}{-2\log(2)}\underset{n\rightarrow\infty}{\lim}\;\frac{2^{\kappa\rho}}{2^{2\rho}}   \\
&= \underset{n\rightarrow\infty}{\lim}\;2^{(\kappa-2)\rho}\\
&=
\begin{cases} 
0 & \text{if $\kappa<2$} \\
1 & \text{if $\kappa=2$} \\
\infty & \text{if $\kappa>2$}
\end{cases}
\enspace,
\end{align*}
where the first two equalities follow from l'H\^opital's rule.

Thus if $\kappa<2$ then $2^{\kappa\rho}$ is $o\left(\left(\log\left(\frac{2^{2\rho}}{2^{2\rho}-1}\right)\right)^{-1}\right)$.

\end{proof}


\begin{remark}
  Note that for a given $\kappa<2$, the lower bound $2^{\kappa\rho}$
  holds only for sufficiently large $\rho(n)$.  By looking at
  Equation~\ref{eqn:zero-label-sample}, and letting $m=2^\rho$,
  we get that $\rho(n)\geq2$ is a sufficient condition for it to hold.  
  If we want a lower bound for robust learning that
  is larger than that of standard learning (where the dependence is
  $\Theta(n)$) for a $\log(n)$ adversary, setting $m=2^{1.7\rho}$
  and requiring $\rho(n)\geq6$, for e.g., would be sufficient.
\end{remark}


\section{Robust Learnability Against a Log-Bounded Adversary}
\label{sec:rob-learning-unif}
The argument showing the non-robust learnability of \MonConj under the uniform distribution in the previous section cannot be carried through if the conjunction lengths are logarithmic in the input dimension, or if the robustness parameter is small compared to that target conjunction's length.
In both cases, we show that it is possible to efficiently robustly learn these conjunctions if the class of distributions is $\alpha$-$\log$-Lipschitz, i.e. there exists  a universal constant $\alpha\geq1$ such that for all $n\in \N$, all distributions $D$ on $\boolhc$ and for all input points $x,x'\in \boolhc$, if $d_H(x,x')=1$, then $|\log(D(x))-\log(D(x'))|\leq\log(\alpha)$ (see Appendix~\ref{app:log-lipschitz} for further details and useful facts).

\begin{theorem}
\label{thm:mon-conj-rob}
  Let $\mathcal{D}=\{\mathcal{D}_n\}_{n\in\mathbb{N}}$, where $\mathcal{D}_n$ is a set of
     $\alpha$-$\log$-Lipschitz distributions on $\{0,1\}^n$ for all $n\in\mathbb{N}$.   Then the class of
    monotone conjunctions is $\rho$-robustly learnable with respect to
    $\mathcal{D}$ for robustness function $\rho(n)=O(\log n)$.
\end{theorem}

The proof can be found in Appendix~\ref{app:mon-conj}.
This combined with Theorem~\ref{thm:mon-conj-rob} shows that $\rho(n)=\log (n)$ is essentially the threshold for efficient robust learnability of the class \MonConj.

The main idea to prove Theorem~\ref{thm:mon-conj-rob} is that, on the one hand, it is possible to efficiently exactly learn the target conjunction if its length is logarithmic in the input dimension.
On the other hand, we can otherwise efficiently $\rho$-robustly learn (but not necessarily exactly learn) longer conjunctions as the robustness parameter is logarithmic in the input dimension, and thus the probability that insufficiently large to cause a label change (with high probability). 
This is quite a simple example that shows that robust learning does not necessarily imply exact learning. 

\begin{proof}

 
  We show that the algorithm $\mathcal{A}$ for PAC-learning monotone
  conjunctions (see \cite{mohri2012foundations}, chapter 2) is a robust learner for an appropriate choice
  of sample size.  We start with the hypothesis $h(x)=\bigwedge_{i\in I_h} x_i$, 
  where $I_h=[n]$. For each example $x$ in $S$, we remove $i$ 
  from $I_h$ if $c(x)=1$ and $x_i=0$.

Let $\D$ be a class of $\alpha$-$\log$-Lipschitz distributions. 
 Let $n\in\mathbb{N}$ and $D\in \mathcal{D}_n$.  Suppose moreover
  that the target concept $c$ is a conjunction of $l$ variables.
  Fix $\varepsilon,\delta>0$. Let $\eta=\frac{1}{1+\alpha}$, 
  and note that by Lemma~\ref{lemma:log-lips-facts},
  for any $S\subseteq[n]$ and $b_S\in\{0,1\}^S$,  we have that 
  $\eta^{|S|}\leq \Pr{x\sim D}{x_i=b}\leq(1-\eta)^{|S|}$.

\paragraph{Claim 1.} 
If
$m \geq \left\lceil \frac{\log n-\log \delta}{\eta^{l+1}}
\right\rceil$ then given a sample $S \sim D^m$, algorithm
$\mathcal{A}$ outputs $c$ with probability at least $1-\delta$.

  \emph{Proof of Claim 1.} Fix $i \in \{1,\ldots,n\}$.  Algorithm
  $\mathcal{A}$ eliminates $i$ from the output hypothesis just in
  case there exists $x\in S$ with $x_{i}=0$ and $c(x)=1$.  Now we
  have $\Pr{x\sim D}{x_{i}=0 \wedge c(x)=1}\geq \eta^{l+1}$
  and hence
\[
\Prob{S\sim D}{\forall  x \in S \cdot i\text{ remains in }I_h}\leq 
(1-\eta^{l+1})^m 
 \leq  e^{-m\eta^{l+1}}
 =  \frac{\delta}{n} \, .
\]
The claim now follows from union bound over $i \in \{1,\ldots,n\}$.

\paragraph{Claim 2.}  If $l \geq \frac{8}{\eta^2}\log(\frac{1}{\varepsilon})$
and $\rho \leq \frac{\eta l}{2}$ then
$\Pr{x\sim D} {\exists z \in B_\rho(x) \cdot c(z)=1}\leq \varepsilon$.

\emph{Proof of Claim 2.}  
Define a random variable $Y=\sum_{i\in I_c} \mathbb{I}(x_i=1)$.  
We simulate $Y$ by the following process. 
Let $X_1,\dots,X_l$ be random variables taking value in $\{0,1\}$, and which may be dependent. 
Let $D_i$ be the marginal distribution on $X_i$ conditioned on $X_1,\dots,X_{i-1}$. 
This distribution is also $\alpha$-$\log$-Lipschitz by Lemma~\ref{lemma:log-lips-facts}, and hence,
\begin{equation}
\label{eqn:marg-bound}
\Pr{X_i\sim D_i}{X_i=1}\leq 1-\eta
\enspace.
\end{equation}

%TODO clean up proof (esp for Y defn), add local smoothness (log lipschitz) definition in mon-conj.tex, appendix with proof of facts, make sure intro is consistent with new proof

%TODO for ITCS version: lemma replacing Claims 1 & 2 (as we reuse Claim 2 for decision lists), add decision list section (after monotone conjunctions), add parity section and mention LMQs there (before monotone conjunctions), amend introduction

Since we are interested in the random variable $Y$ representing the number of 1's in $X_1,\dots,X_l$, 
we define the random variables $Z_1,\dots,Z_l$ as follows:
\begin{equation*}
Z_k = \left(\sum_{i=1}^k X_i\right)-k(1-\eta)\enspace.
\end{equation*} 
The sequence $Z_1, \dots, Z_l$ is a supermartingale with respect to $X_1,\dots,X_l$:
\begin{align*}
\eval{}{Z_{k+1}\given X_1,\dots,X_k}
&=\eval{}{Z_{k}+X_{k+1}'-(1-\eta)\given X'_1,\dots,X'_k}\\
%&=Z_k+\eval{}{\mathbf{1}[X_{k+1}'=1]\given X'_1,\dots,X'_k}-(1-\eta)\\
&=Z_k+\Pr{}{X_{k+1}'=1\given X'_1,\dots,X'_k}-(1-\eta)\\
&\leq Z_k
\enspace. \tag{by (\ref{eqn:marg-bound})}
\end{align*}
Now, note that all $Z_k$'s satisfy $|Z_{k+1}-Z_k|\leq 1$, and that $Z_l=Y-l(1-\eta)$. 
We can thus apply the Azuma-Hoeffding (A.H.) Inequality to get 
\begin{align*}
\Pr{}{Y\geq l-\rho}
&\leq \Pr{}{Y\geq l(1-\eta)+\sqrt{2\ln(1/\varepsilon)l}}	\\
&=\Pr{}{Z_l-Z_0\geq \sqrt{2\ln(1/\varepsilon)l}}	\\
&\leq \exp\left(-\frac{\sqrt{2\ln(1/\varepsilon)l}^2}{2l}\right)				\tag{A.H.}\\
&=\varepsilon
\enspace,
\end{align*}
where the first inequality holds from the given bounds on $l$ and $\rho$:
\begin{align*}
l-\rho &=(1-\eta)l + \frac{\eta l}{2} 
               + \frac{\eta l}{2} - \rho \\
          & \geq (1-\eta) l + \frac{\eta l}{2} 
           \tag{since $\rho \leq \frac{\eta l}{2}$}\\
          & \geq  (1-\eta) l + \sqrt{2\log(1/\varepsilon) l} \enspace.
            \tag{since $l \geq \frac{8}{\eta^2}\log(\frac{1}{\varepsilon})$}
\end{align*}
This completes the proof of Claim 2.

We now combine Claims 1 and 2 to prove the theorem.  Define
$l_0 := \max(\frac{2}{\eta}\log n,
\frac{8}{\eta^2}\log(\frac{1}{\varepsilon}))$.  Define
$m:=\left\lceil \frac{\log n-\log \delta}{\eta^{l_0+1}}
\right\rceil$.  Note that $m$ is polynomial in $n$, $\delta$,
$\varepsilon$.  

Let $h$ denote the output of algorithm $\mathcal{A}$ given a sample
$S\sim D^m$.  We consider two cases.  If $l \leq l_0$ then, by
Claim 1, $h=c$ (and hence the robust risk is $0$) with probability at
least $1-\delta$.  If $l_0 \leq l$ then, since $\rho=\log n$, we
have $l \geq \frac{8}{\eta^2}\log(\frac{1}{\varepsilon})$ and
$\rho \leq \frac{\eta l}{2}$ and so we can apply Claim 2.  By Claim
2 we have
\[ \roblosse(h,c) \leq \Pr{x\sim D}{\exists z \in B_\rho(x) \cdot c(z)=1} \leq \varepsilon \]

\end{proof}



